Now you see it, Now you don't: Damage Label Agreement in Drone & Satellite Post-Disaster Imagery

This paper audits damage labels derived from coincident satellite and drone aerial imagery for 15,814 buildings across Hurricanes Ian, Michael, and Harvey, finding 29.02% label disagreement and significantly different distributions between the two sources, which presents risks and potential harms during the deployment of machine learning damage assessment systems. Currently, there is no known study of label agreement between drone and satellite imagery for building damage assessment. The only prior work that could be used to infer if such imagery-derived labels agree is limited by differing damage label schemas, misaligned building locations, and low data quantities. This work overcomes these limitations by comparing damage labels using the same damage label schemas and building locations from three hurricanes, with the 15,814 buildings representing 19.05 times more buildings considered than the most relevant prior work. The analysis finds satellite-derived labels significantly under-report damage by at least 20.43% compared to drone-derived labels (p<1.2x10^-117), and satellite- and drone-derived labels represent significantly different distributions (p<5.1x10^-175). This indicates that computer vision and machine learning (CV/ML) models trained on at least one of these distributions will misrepresent actual conditions, as the differing satellite and drone-derived distributions cannot simultaneously represent the distribution of actual conditions in a scene. This potential misrepresentation poses ethical risks and potential societal harm if not managed. To reduce the risk of future societal harms, this paper offers four recommendations to improve reliability and transparency to decisio-makers when deploying CV/ML damage assessment systems in practice

==> Facct25/sections/deprecated/introduction_v1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Facct25/Figures/suas_vs_satellite_reformatted.png}
    \caption{Three buildings with different damage labels in different views between drone (top-row) and satellite (bottom-row) aerial imagery. [Left Column] Label change due to changing flood waters. [Middle Column] Label change due to debris removal. [Right Column] Label change due to roof repairs.}
    \label{fig:suas-vs-satellite}
\end{figure}

The potential benefits of aerial imagery for disaster assessment rely on the correct interpretation of that imagery; a 2024 National Academies of Sciences Engineering and Medicine study\cite{NASGCC:24} described how mislabeled UAS imagery in the aftermath of Hurricane Laura in Lake Charles, Louisiana, caused repairable houses to be demolished and ultimately led to local agencies rejecting the use of virtual inspections for future events. 
%Todo introduce satellite and drone imagery before aerial imagery
%Introduce label agreement/disagreement
%Explain why we chose the hurricanes/disasters we did
%risks and harms when 

However, until this point, the computer vision and machine learning (CV/ML) literature has assumed that labels derived from aerial imagery can accurately represent disaster scenes such labels can be used to perform automated damage assessments in hopes of delivering a positive impact on disaster response operations \cite{robinson2023rapid, gupta2019creating, rahnemoonfar2021floodnet, rahnemoonfar2022rescuenet, zhu2021msnet, cheng2021dorianet, IdaBDDataset, manzini2024crasar, haitiBRDDataset, liuLargeScale2019, chen2018benchmark, fujita2017damage, Pi2020, IanBD, chen2025bright}. 
This assumption has been unchallenged, and there has not been an effort to determine if aerial imagery-derived labels are a consistent source of information for automated damage assessments and, most importantly, if aerial imagery-derived labels used to train and evaluate automated damage assessment systems can represent the distribution of damage present in a disaster scene.

To challenge this assumption and to measure the potential for errors in post-disaster aerial imagery-based damage assessment, this work audits differences in labels derived from coincident drone and satellite aerial imagery for 15,812 buildings from Hurricanes Ian, Michael, and Harvey. 
Any instances where label disagreement occurs between drone and satellite are indicative of the label disagreement that may be observed in practice. When label disagreement occurs between satellite and drone views, it is unclear which labels will represent the actual conditions present in the scene and, as a result, represent instances of misclassifications that may lead to societal harm as observed in \cite{NASGCC:24}. Examples of disagreements within this coincident imagery are shown in Figure \ref{fig:suas-vs-satellite}. 

%The capacity for aerial imagery-based damage assessments to deliver operational impact depends entirely on the accuracy of the assessment.
    
The core contribution of this work is a data audit in the form of a statistical comparison of damage labels derived from coincident satellite and drone aerial imagery for 15,812 buildings across Hurricanes Ian,
Michael, and Harvey. This work overcomes the limitations of the most relevant prior work \cite{robinson2023rapid} by comparing 19.05 times more buildings, using the same damage scale and the same building locations.

The terminology referenced in this work is defined as follows. Drone-derived labels are defined as human-sourced and curated labels of imagery generated based on observations of imagery collected by a drone. Satellite-derived labels are the same as drone-derived labels, only having their labels based on imagery collected by satellites. Aerial imagery-derived labels represent labels that are derived from any aerial view, including satellites, drones, or other sources. Finally, ground-level labels refer to labels that are generated based on a determinative in-situ human assessment.

This document begins with a discussion of the related work in Section \ref{sec:related-work}, followed by a summary of the approach used to collect, label, and curate the data for this audit in Section \ref{sec:approach}, describes the analysis techniques used and results found in Section \ref{sec:analysis}, provides a discussion of the analysis and results in Section \ref{sec:discussion}, and concludes in Section \ref{sec:conclusion} with a summary, recommendations, and discussion of future work.


